Mixture of Experts in a Mixture of RL settings

Mixtures of Experts (MoEs) have gained prominence in (self-)supervised learning due to their enhanced inference efficiency, adaptability to distributed training, and modularity. Previous research has illustrated that MoEs can significantly boost Deep Reinforcement Learning (DRL) performance by expanding the network's parameter count while reducing dormant neurons, thereby enhancing the model's learning capacity and ability to deal with non-stationarity. In this work, we shed more light on MoEs' ability to deal with non-stationarity and investigate MoEs in DRL settings with "amplified" non-stationarity via multi-task training, providing further evidence that MoEs improve learning capacity. In contrast to previous work, our multi-task results allow us to better understand the underlying causes for the beneficial effect of MoE in DRL training, the impact of the various MoE components, and insights into how best to incorporate them in actor-critic-based DRL networks. Finally, we also confirm results from previous work.

==> oldStructure.tex <==

\begin{abstract}


Mixture of Experts (MoEs), a type of neural network layer, comprising multiple expert units and a router module that directs tokens to these experts, has gained prominence in (self-) supervised learning due to their enhanced inference efficiency, adaptability to distributed training, and their ability to specialise. Their modular design allows for distinct focuses such as coding or language processing in Large Language Models (LLMs). Previous research has illustrated that MoEs can significantly boost Deep Reinforcement Learning (DRL) performance by expanding the network's parameter count while simultaneously reducing dormant neurons, thereby enhancing the model's learning capacity. Our study reveals that the augmented capacity provided by MoEs benefits DRL and proves advantageous in multi-task RL and continual RL scenarios, where managing learning capacity is crucial. Furthermore, we conduct an in-depth analysis of various router modules and architectures within MoEs. We offer insights into best practices for their integration into DRL systems, thereby contributing to a more nuanced understanding of how MoEs can optimize DRL performance across various settings.
\end{abstract}

\section{Introduction}
\label{sec:introduction}


Deep Reinforcement Learning (RL), which integrates reinforcement learning algorithms with deep neural networks, demonstrated remarkable success in enabling agents to achieve complex tasks beyond human capabilities in domains ranging from video games to strategic board games and beyond \citep{mnih2015humanlevel, berner2019dota, vinyals2019grandmaster, fawzi2022discovering, Bellemare2020AutonomousNO}. Despite the pivotal role of deep networks in these advanced RL applications, the intricacies of their design and the mechanisms of their learning processes within RL contexts are not fully understood. Intriguingly, recent research has uncovered unexpected behaviours and phenomena associated with the use of deep networks in RL, which often diverge from those observed in traditional supervised learning environments \citep{ostrovski2021tandem,kumar2021implicit, lyle2022understanding,graesser2022state,nikishin22primacy,sokar2023dormant,ceron2023small}.


Significant architectural innovations, such as transformers \citep{vaswani2017attention}, adapters \citep{houlsby19parameter}, and Mixture of Experts \citep[MoEs;][]{shazeer2017outrageously}, have played a pivotal role in the scalability of supervised learning models, particularly within the domains of natural language processing and computer vision. MoEs stand out in their ability to facilitate the scaling of networks to encompass billions and even trillions of parameters, a feat made possible through their modular design that seamlessly integrates with distributed computing techniques~\citep{fedus2022switch}. Moreover, MoEs introduce a form of structured sparsity into the network architecture, a characteristic associated with enhancements in network performance through various studies on network sparsity \citep{evci2020rigl,gale2019state,jin2022pruning}.

Multi-Task Reinforcement Learning (MTRL) and Continual Reinforcement Learning (CRL) have emerged as compelling frameworks for probing the limitations inherent in Deep Reinforcement Learning (DRL)\citep{calandriello2014sparse, khetarpal2022towards}. These paradigms accentuate the challenges of DRL, such as catastrophic forgetting, inefficient parameter utilization, and the difficulty of transferring knowledge across diverse contexts. MTRL and CRL demand that agents generalize across multiple tasks or adapt to new tasks over time without forgetting previous knowledge. Previous research within these domains has been instrumental in identifying and addressing these shortcomings, proposing methods enhancing learning efficiency, improving memory retention, and facilitating knowledge transfer \citep{calandriello2014sparse,devin2017learning,yang2020multi,sun2022paco,deramo2024sharing}. 

%Rather than proposing new MTRL or Continual RL methodologies, our investigation leverages these settings to explicitly evaluate MoEs for DRL on prevalent challenges in deep Reinforcement Learning (RL), such as capacity loss, dormant neurons, and catastrophic forgetting. By applying a Mixture of Experts (MoE) approach within the MTRL and Continual RL context, where these problems are accentuated, we aim to provide a better understanding of MoES for DRL.
We focus on evaluating the potential of MoEs to address core DRL challenges: capacity loss, dormant neurons, and catastrophic forgetting. 
These challenges are accentuated in MTRL and Continual RL methods, both of which we use as a testbed showing how MoEs might optimize DRL performance.

We conduct a comprehensive investigation into possibilities for integrating Mixture of Experts (MoEs) within actor-critic-based DRL architectures, focusing on the placement of MoE layers, the architecture of experts, and types of routers. In contrast to prior work \citep{obando2024mixtures}, our work provides an in-depth analysis of routing decisions, uncovering that, in some cases, MoEs specialise in the final layers while learning joint representations in the initial layers. %We also showcase how some results transfer to the single environment case. 
Through this exploration, we shed light on the potential of MoEs to enhance the effectiveness of DRL agents across a spectrum of learning tasks and environments and reproduce positive results from prior work on value-based methods.


\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{figures/architectures/bigMoEs.pdf}
    \caption{\textbf{Architectures considered: (a)} Baseline architecture; \textbf{(b)} \middlemoe,  used by \citet{obando2024mixtures}; \textbf{(c)} \finalmoe, where the final layer is replaced by an MoE module; \textbf{(d)} \allmoe, where all layers are replaced with an MoE module; \textbf{(c)} \bigmoe, with a single MoE module where an expert comprises the full original network.}
    \label{fig:moe_architectures}
    \vspace{-0.5em}
\end{figure}


\section{Background}
\subsection{Reinforcement Learning}
A Markov Decision Process \citep[MDP]{bellman1957markovian, puterman1990markov, sutton2018reinforcement} consists of a tuple $\mathcal{M}=\langle\mathcal{S}, \mathcal{A}, \mathcal{P}, r, \rho, \gamma\rangle$. Here, $\mathcal{S}$ denotes the set of all possible states, $\mathcal{A}$ represents the set of possible actions, and $\mathcal{P}: \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ defines the probability distribution of transitioning to state $s'$ from state $s$ after taking action $a$. The function $r: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ specifies the reward received after taking an action $a$ in state $s$, $\rho$ describes the initial state distribution, and $\gamma$ (where $0 < \gamma \leq 1$) is the discount factor that determines the present value of future rewards. In Reinforcement Learning (RL), a policy $\pi$ assigns to each state $s$ a probability distribution over actions in $\mathcal{A}$. The objective in RL is to devise a policy $\pi$ that maximizes the expected sum of discounted rewards $J(\pi)=\mathbb{E}_\pi\left[\sum_{t=0}^{\infty} \gamma^t r\left(s_t, a_t\right)\right]$. The policy parameterized by $\theta$ is denoted as $\pi_\theta(a_t \mid s_t)$.
%is parameterized by $\theta$.
The parameter $\theta$ is chosen via optimization maximizing $J(\theta)$, thereby achieving the highest possible cumulative reward.

In \textbf{Multi-Task Reinforcement Learning} (MTRL), an agent engages with a variety of tasks $\tau$ from a set $\mathcal{T}$, with each task $\tau$ constituting a distinct Markov Decision Process (MDP) denoted by $\mathcal{M}^\tau = \langle \mathcal{S}^\tau, \mathcal{A}^\tau, \mathcal{P}^\tau, r^\tau, \rho^\tau, \gamma^\tau \rangle$. The objective in MTRL is to devise a unified policy $\pi$ that optimizes the average expected cumulative discounted return across all tasks, expressed as $J(\theta) = \sum_\tau J_\tau(\theta)$. The tasks may vary across one or several MDP components, with task-specific information being provided either through a task identifier, like a one-hot vector, or via metadata, such as a task description, following the approach by \citet{sodhani2021multi}.

For \textbf{Continual RL}, following \citet{abbas2023loss}, we focus on a specific setting of Continual RL, where the agent plays a fixed sequence of MDPs for a fixed number of steps respectively and will revisit said MDPs in the same order, e.g., we have two MDPs ($\mathcal{M}^1$, $\mathcal{M}^2$) and train on a sequence such as $\mathcal{M}^1\rightarrow\mathcal{M}^2\rightarrow\mathcal{M}^1\rightarrow\mathcal{M}^2$. By revisiting the MDPs, we evaluate the agent's capacity to remember or relearn strategies.

\begin{figure*}[t]
    \centering
    % \includegraphics[width=\textwidth]{figures/continual_rl/top/crl_learning_curve.png}
    % \includegraphics[width=\textwidth]{figures/continual_rl/top/crl_top.png}
    \includegraphics[width=\textwidth]{figures/Continual_CTRL2.pdf}
    \caption{\textbf{Comparison of different models and routers on the continual RL setup}. We report the learning curve scores for 3 Atari games. All games run with 10 independent seeds, shaded areas representing 95\% confidence intervals. BigMoE improves performance over the baseline across all the games.\vspace{-3mm}}
    \label{fig:crl_top}
    \vspace{-0.5em}
\end{figure*}



\subsection{MoEs}
\label{sec:moeBackground}
Mixtures of Experts (MoEs) have emerged as a cornerstone in the design of Large Language Models (LLMs), integrating a collection of $n$ ``expert'' sub-networks. 
A gating mechanism, known as the router and usually learned during training, manages the experts by directing each incoming token to $k$ selected experts \citep{shazeer2017outrageously}. Typically, $k$ is less than the total count of experts (in our case, $k=1$). This sparsity is key for enhancing inference speed and facilitating distributed computing, making it a pivotal factor in training LLMs. In transformer architectures, MoE units substitute all dense feedforward layers \citep{vaswani2017attention}. The impressive empirical performance of MoEs has sparked significant research interest \citep{shazeer2017outrageously,Lewis2021BASELS,fedus2022switch,zhou2022mixture,puigcerver2023sparse,lepikhin2020gshard,zoph2022stmoe,gale2023megablocks}.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/netsModel.pdf}
    \caption{\textbf{Models: ...}}
    \label{fig:a}
\end{figure*}

The strict routing of tokens to specific experts, known as hard assignments, presents several issues, including training instability, token loss, and obstacles in expanding the number of experts \citep{fedus2022switch,puigcerver2023sparse}. To mitigate these issues, \citet{puigcerver2023sparse} proposed the concept of \textbf{Soft MoE}, which utilizes a soft, fully differentiable method for allocating tokens to experts, thereby circumventing the limitations associated with router-based hard assignments. This soft assignment method calculates a blend of weights for each token across the experts and aggregates their outputs accordingly. 
Adopting \citet{puigcerver2023sparse} terminology, consider input tokens represented by $ \mathbf{X} \in \mathbb{R}^{m \times d} $, with $ m $ indicating the count of $ d $-dimensional tokens. A Soft MoE layer processes these tokens through $ n $ experts, each defined as $ \{f_i: \mathbb{R}^d \rightarrow \mathbb{R}^d\}_{1: n} $. Every expert is associated with $ p $ slots for both input and output, each slot characterized by a $ d $-dimensional vector of parameters. These parameters are collectively denoted as $ \boldsymbol{\Phi} \in \mathbb{R}^{d \times(n \cdot p)} $.

The input slots $\tilde{\mathbf{X}} \in \mathbb{R}^{(n \cdot p) \times d}$ represent a weighted average of all tokens, given by $\tilde{\mathbf{X}}=\mathbf{D}^{\top} \mathbf{X}$, where $\mathbf{D}$ is commonly known as the dispatch weights. The outputs from the experts are expressed as $ \tilde{\mathbf{Y}}_i = f_{\lfloor i / p\rfloor}(\tilde{\mathbf{X}}_i) $. For the Soft MoE layer, the overall output $ \mathbf{Y} $ results from merging $ \tilde{\mathbf{Y}} $ with the combined weights $ \mathbf{C} $, described by $ \mathbf{Y} = \mathbf{C} \tilde{\mathbf{Y}} $. $\mathbf{D}$ and $\mathbf{C}$ are represented by the following expressions: 


\sidebysideequations[0.6]{
            \mathbf{D}_{i j}=\frac{\exp \left((\mathbf{X} \boldsymbol{\Phi})_{i j}\right)}{\sum_{i^{\prime}=1}^m \exp \left((\mathbf{X} \boldsymbol{\Phi})_{i^{\prime} j}\right)}. \notag
            }{\mathbf{C}_{i j}=\frac{\exp \left((\mathbf{X} \boldsymbol{\Phi})_{i j}\right)}{\sum_{j^{\prime}=1}^{n \cdot p} \exp \left((\mathbf{X} \boldsymbol{\Phi})_{i j^{\prime}}\right)} \notag
            }
The findings from \citet{puigcerver2023sparse} indicate that Soft MoE provides an improved balance between accuracy and computational expense relative to alternative MoE approaches.


\section{Experiments}

% Why continual RL? Why multi-task RL?

This paper focuses on investigating the potential performance benefits of MoEs within DRL, rather than proposing a novel DRL method for MTRL or Continual RL. We hypothesize that MoEs, with their modular nature, address general DRL weaknesses such as capacity loss, dormant neurons, and catastrophic forgetting \citep{sokar2023dormant, abbas2023loss}. We evaluate this hypothesis within MTRL and Continual RL, as these settings accentuate those weaknesses. Improvements observed here would suggest the potential for wider gains in single-environment DRL.

Our agents are trained with Proximal Policy Optimisation \citep[PPO]{schulman2017proximal}, in contrast to \citet{obando2024mixtures} that use value-based methods. We rely on the Gymnax suite \citep{gymnax2022github} to implement our MinAtar environments \citep{young19minatar}. The PPO implementation is based on the PureJaxRL codebase\footnote{PureJaxRL code available at: \href{https://github.com/luchris429/purejaxrl}{https://github.com/luchris429/purejaxrl}} \citep{lu2022model, lu2022discovered, lu2023adversarial}. Hyperparameters are provided in \autoref{app:hps} and were adapted from \citet{jesson2023relu}. We only deviate in the network size due to computational constraints. For all experiments, we evaluate on three environments: SpaceInvaders (SI), Breakout (BO), and Asterix (Ast). Asterix visually differs substantially from SpaceInvaders and Breakout, whereas the latter two are similar in observation and action space. This environment selection allows us to investigate whether MDP similarity encourages sharing representations between experts.
%and comparison among methods across varying environments


\begin{figure}[!t]
    \centering
     \includegraphics[width=0.3\textwidth]{figures/cosineSim.pdf}%
   \vline height 95pt depth 0 pt width 1.2 pt
   \includegraphics[width=0.7\textwidth]{figures/SoftGradientMOEs2.pdf}%
   \caption{\textbf{Left:} Display the sequential gradient similarity calculated whenever a bucket is full. This corresponds to the diagonal of the heatmap. \textbf{Right:} Results with gradient-based MoE.}
   \label{fig:gradient_analysis}
   \vspace{-1em}
\end{figure}

In our \textbf{Continual RL} setup, we train the agent on a fixed sequence of MDPs for a fixed amount of environment steps respectively, akin to \citep{abbas2023loss}. Specifically, the agent trains on SI $\rightarrow$ BO $\rightarrow$ Ast $\rightarrow$ SI $\rightarrow$ BO $\rightarrow$ Ast. By revisiting MDPs, we evaluate whether the agent relearns the policy once more (learning capacity) or retains the policy and performs well out of the gate (memorisation). For \textbf{MTRL}, We train simultaneously on SI, BO, and Ast. In practice, the PPO agent performs one update step per environment right after each other. Finally, we train in a \textbf{single environment} setting, where we train our agents on SpaceInvaders, Breakout and Asterix individually to test if any of the findings from our MTLR and Continual RL settings transfer to the single environment case.

In our experiments, we implement four different variants of MoEs. \citet{obando2024mixtures} propose to replace the penultimate layer with an MoE module and keep the other layers shared across the network. We term this variant \middlemoe. Similarly, we also evaluate a variant called \finalmoe, where the MoE module replaces the last layer. Inspired by our experiments that parameter sharing might be detrimental, we also propose two new architectures, \allmoe and \bigmoe. In \allmoe, all three layers are replaced by MoE modules. In \bigmoe, the network contains a single MoE module and each expert consists of a full network, i.e., three layers. For a visualisation, see \autoref{fig:moe_architectures}. All hyperparameters are reported in \autoref{app:hyperparams}.

\section{Results}
\subsection{Continual RL}

\paragraph{Hardcoded routers under parameter sharing.}
% If we know exactly when to switch, does it improve performance? -> We introduce the Hardcoded Router. -> Doesn't work when sharing parameters
We first experiment in an idealized scenario where the router has perfect information of which task the data is coming from, and routes to the according per-task expert.
We refer to this as a Hardcoded Router. 
Such routing allows us to decouple router learning-related and expert architecture-related performance changes in continual RL.
%Exploring the potential of precise timing in switching between tasks, we introduce the concept of the Hardcoded Router to determine whether a pre-defined schedule for task transitions can enhance model performance. 
The Hardcoded Router routes observations solely based on the task identifier. 
We first evaluate \middlemoe and \finalmoe architectures which have shared parameters among the tasks.
%parameter sharing. 
As shown in \autoref{fig:crl_shared_params} and \autoref{tab:crl_shared_params}, the Hardcoded Router does not improve performance drastically in these MoE architecture variations with parameter sharing, e.g., (0.52 $\pm$ 0.01 vs. 0.46 $\pm$ 0.03) for \middlemoe and baseline respectively.
%in scenarios where parameters are shared between experts.

% % Maybe parameter sharing is the problem? -> We introduce BigMoE and AllLayers variants. % Now hardcoded works very well
\paragraph{Hardcoded routers under complete modularity.}
The results reported above raise a question whether parameter sharing is detrimental in MoE architectures for Continual RL.
%led us to hypothesize that parameter-sharing might be detrimental. 
To investigate this further, we propose and test two new MoE architecture variants: \bigmoe and \allmoe, where no parameters are shared among experts. 
The results in \autoref{fig:crl_isolated_params} and \autoref{tab:crl_isolated} demonstrate that Hardcoded Router exhibits significantly improved performance for \bigmoe (0.67 $\pm$ 0.02) and \allmoe (0.56 $\pm$ 0.02) architectures as compared to \middlemoe (0.52 $\pm$ 0.01) and \finalmoe (0.42 $\pm$ 0.02). 

%The Hardcoded Router approach exhibits significantly improved performance with these adjustments, suggesting that the architecture's adaptability to task switching is crucial, see \cref{fig:crl_hardcoded_noparam_sharing}.

% Can learned routers achieve the same? -> No but not expected. Hard to learn for router. 
Despite the success of hardcoded routing, the question arises: Can learned routers, which dynamically determine task switches, achieve comparable results? Our experiments indicate that learned routers (e.g., \bigmoe-SoftMoE) do not match the performance of their hardcoded counterparts (0.67 $\pm$ 0.02, 0.53 $\pm$ 0.02), as shown in \autoref{fig:crl_top}. However, \bigmoe-SoftMoE performs better than the baseline (0.53 $\pm$ 0.02, 0.46 $\pm$ 0.03) (see \autoref{tab:crl_top}), whereas \bigmoe-TopK does not (0.39 $\pm$ 0.02, 0.46 $\pm$ 0.03). For all results, please see the Appendix \ref{app:mtrl_more_results}, \ref{app:crl_more_results} and \ref{app:single_env_more_results}.

\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Game & Baseline & \bigmoe-Hardcoded & \bigmoe-TopK & \bigmoe-SoftMoE \\
\hline
SI & 0.97 \pm 0.01 & 0.95 \pm 0.00 & 0.90 \pm 0.01 & 0.98 \pm 0.01 \\
BO & 0.08 \pm 0.05 & 0.32 \pm 0.03 & 0.13 \pm 0.02 & 0.08 \pm 0.03 \\
Ast & 0.35 \pm 0.04 & 0.56 \pm 0.04 & 0.20 \pm 0.01 & 0.46 \pm 0.03 \\
SI-2 & 0.78 \pm 0.12 & 0.97 \pm 0.00 & 0.75 \pm 0.12 & 0.82 \pm 0.13 \\
BO-2 & 0.08 \pm 0.02 & 0.34 \pm 0.04 & 0.02 \pm 0.01 & 0.13 \pm 0.03 \\
Ast-2 & 0.52 \pm 0.06 & 0.85 \pm 0.05 & 0.35 \pm 0.01 & 0.72 \pm 0.03 \\
\hline
Total & 0.46 \pm 0.03 & \textbf{0.67} \pm 0.02 & 0.39 \pm 0.02 & 0.53 \pm 0.02 \\
\hline
\end{tabular}
\caption{Continual RL: Normalised Performance of algorithms across games. For the average performance, we report the mean and standard error over 10 seeds of the average performance across environments. We normalise performance according to the single environment results reported in \citet{jesson2023relu}.}
\label{tab:crl_top}
\end{table}

\paragraph{Learning routers based on task id and gradient signal.}
% What if we give task id as input? -> Still doesn't work 
The results above indicate that, given a router that can perfectly distinguish among the tasks, MoE architectures without parameter sharing may bring performance benefits.
These results, however, rely on the oracle Hardcoded Router. 
Here we investigate how well a router can be learned. We evaluate multiple learning signals: gradient-based and even task ids, all of which yield mixed results. 

%In light of these findings, we explored whether providing the task identifier as an additional input to the model could facilitate the learning process for routers.
We first evaluate a case where a task id is given as an input, reported in \autoref{fig:crl_task_id} and \autoref{tab:crl_task_id}. 
Surprisingly, we found that learning a router based on the task id resulted in a performance drop relative to the learned router version without task id (0.53 $\pm$ 0.02, 0.47 $\pm$ 0.02).
%Surprisingly, this approach did not improve performance,
These results suggest that more than the mere inclusion of task identifiers is needed for routers to learn task-switching strategies effectively.

% Can we add additional information to help with switching? -> Gradient Analysis % Point to Heatmap of gradient similarity
We next evaluate other task-dependent signals to facilitate learning a router. 
Intuitively, when a task switches, the network's gradients might change abruptly. 
By examining the similarity of gradients across different tasks, we aim to identify patterns that could inform more strategic task switching. We analyse gradient similarity by bucketing the gradients along training and comparing the cosine similarity of the buckets (representing the average of all gradients in that bucket). As shown in \autoref{fig:gradient_analysis}, the gradient similarity does decrease whenever the MDP switches.

% What if we switch based on gradient diff? -> Hard to find hyperparameters that help 
Experimenting with gradient differences as a basis for switching tasks presented challenges, primarily in identifying the optimal gradient difference threshold. For example, \autoref{fig:crl_grad_switch} shows that the model might already switch in the first visit of SpaceInvaders, shown by the two dips in training.

% What if we just add gradient diff information as input? -> Doesn't really learn
Instead, we incorporate gradient difference information directly as an input to the model.
%, hypothesizing that this could enhance the router's ability to make informed decisions. 
However, our results in \autoref{fig:softgradmoe} and \autoref{tab:crl_softgradmoe} show no improvements in performance (0.53 $\pm$ 0.02, 0.53 $\pm$ 0.02), indicating that simply adding gradient difference data as input does not sufficiently equip the model to learn effective task-switching strategies. Our findings suggest that learning a router in continual RL is extremely challenging, which we hypothesize is due to too-infrequent and too-few task switches which provide the critical data for router learning.

\begin{figure*}[t]
    \centering
    % \includegraphics[width=\textwidth]{figures/multi_task/top/mtrl_learning_curve.png}
    % \includegraphics[width=\textwidth]{figures/multi_task/top/mtrl_top.png}
    \includegraphics[width=\textwidth]{figures/Continual_MTRL2.pdf}
    \caption{\textbf{Comparison of different models and routers on the multi-task setup}. We report the learning curve scores for 3 Atari games. All games run with 10 independent seeds, shaded areas representing 95\% confidence intervals. BigMoE improves performance over the baseline, especially due to performance improvements in SpaceInvaders and Asterix.\vspace{-2mm}}
    \label{fig:mtrl_top}
\end{figure*}

\subsection{Multi-Task RL}

%% Maybe easier to learn to switch since router gets task information simultaneously. % Do Hardcoded Routers help? -> not really out of the gate, doesn't matter if parameters are shared or not
%In MTRL, routers can more easily discern how to route between experts as they are trained on all tasks simultaneously. However, Hardcoded Routers do not improve performance, regardless of whether parameters are shared across tasks, as shown in \cref{fig:mtrl_hardcoded_all_architectures}.

In contrast to a continual setting, we hypothesize that in MTRL routers should be easier to learn due to simultaneous training across all tasks, giving the router a lot more signal for learning.
In this section, we evaluate this hypothesis: we attempt to learn all routers, compare router learning to router hardcoding, and evaluate the combination of the two. 

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Game & Baseline & \bigmoe-Hardcoded & \bigmoe-TopK & \bigmoe-SoftMoE \\
\hline
SI & 0.90 \pm 0.01 & 0.95 \pm 0.01 & 0.90 \pm 0.01 & 0.93 \pm 0.01 \\
BO & 0.46 \pm 0.07 & 0.57 \pm 0.07 & 0.30 \pm 0.02 & 0.60 \pm 0.09 \\
Ast & 0.51 \pm 0.05 & 0.59 \pm 0.01 & 0.33 \pm 0.03 & 0.62 \pm 0.05 \\
\hline
Total & 0.63 \pm 0.03 & \textbf{0.70} \pm 0.02 & 0.51 \pm 0.02 & \textbf{0.72} \pm 0.03 \\
\hline
\end{tabular}
\caption{Multi-Task reinforcement learning: Normalised Performance of algorithms across games with average total performance. We normalise performance according to the single environment results reported in \citet{jesson2023relu}.}
\label{tab:mtrl_top}
\end{table}

\paragraph{Learned Soft Routers compared to Hardcoded Routers.} 
% But maybe learned routers help? -> Help a little but not so much 
% What do they learn -> AllLayers analysis
% It specialises in the final layer and learns shared representations in earlier layers but performance not better
Learned routers improve over the baseline (0.72 $\pm$ 0.03, 0.63 $\pm$ 0.03) \textit{and} and perform as well as a hardcoded router (0.72 $\pm$ 0.03, 0.70 $\pm$ 0.02), see \autoref{fig:mtrl_top} and \autoref{tab:mtrl_top}. This prompts a deeper examination of what these routers are learning. Analysis of the \allmoe-SoftMoE variant reveals that there is a tendency for specialization in the final layer, as shown in \autoref{fig:mtrl_expert}, with shared representations being more common in earlier layers. The final layer tends to prefer specific experts per task. Interestingly, for SI and BO, which are similar MDPs, the same experts are chosen, whereas for Asterix, a distinct combination of experts is preferred. However, as shown in \autoref{fig:mtrl_smsmhc}, this configuration does not translate into superior performance over the baseline. \bigmoe-SoftMoE also displays task specialisation (see \autoref{fig:mtrl_big_expert})


\paragraph{Combining router learning with some task-specialized layers via Hardcoding.}
% Do we expect final layer specialisation to help? -> We introduce SMSMHC (SoftMoE, SoftMoE, Hardcoded Router), where first two layers are learned SoftMoE layers and last layer is a Hardcoded Router -> Doesn't help performance
Building on the result above, we test how enforced task-specialization in the final layer affects performance. 
For this, we introduce a new architecture termed SMSMHC (SoftMoE, SoftMoE, Hardcoded Router).
%to test whether final layer specialization can be beneficial. 
This architecture consists of two initial layers of learned SoftMoE and a final layer with a Hardcoded Router. Contrary to expectations, SMSMHC does not yield a performance improvement ( 0.56 $\pm$ 0.02 & 0.53 $\pm$ 0.01), as shown in \autoref{fig:mtrl_smsmhc}, leading to questions about the value of specialization in this context.

\paragraph{Increasing routing entropy.}
% If specialisation does not help, maybe we should encourage it to route more randomly -> entropy regularisation -> doesn't really help
Given the limited success of specialization, we hypothesize that encouraging more random routing via entropy regularization might help.  
%we encourage more random routing by regularising the entropy of the router. 
Unfortunately, this approach also falls short, failing to produce a meaningful enhancement in performance for \bigmoe-SoftMoE (0.70 $\pm$ 0.02 & 0.72 $\pm$ 0.03) and \allmoe-SoftMoE (0.55 $\pm$ 0.02 & 0.56 $\pm$ 0.02). See \autoref{fig:mtrl_re} and \autoref{tab:mtrl_re}.
The expert selection probabilities are shown in Figure \ref{fig:mtrl_big_expert} and \ref{fig:mtrl_expert}.

\paragraph{MoE effect on dormant neurons.}
% Maybe dormant neurons is the culprit
\citet{obando2024mixtures} suggest that using MoEs in value-based networks lowers dormant neurons. The authors hypothesize that the reduce in dormant neurons might explain the performance benefits observed in single environment RL. MoEs also reduce dormant neurons in MTRL (see \autoref{fig:mtrl_dormant}) and CRL (see \autoref{fig:crl_dormant}).
%As we do not observe strict performance improvements in MTRL, we also analyse dormant neurons and show that they are indeed lower than the baseline, confirming the previous result for actor-critic based methods, see \cref{fig:mtrl_dormant_neurons}. However, our results suggest that low dormant neurons does not lead to performance improvement.

\paragraph{Implications for single-environment RL.}
% Can we transfer any of our findings to single env
This series of experiments, spanning various configurations and strategies, opens the door to reflecting on the transferability of these insights to single-environment settings. Despite the challenges and mixed outcomes, the exploration sheds light on the complexities of designing effective routing mechanisms in multi-task learning systems, paving the way for further research into optimizing task switching and information processing within such models.


\begin{figure*}[t]
    \centering
    % \includegraphics[width=\textwidth]{figures/single_env/top/single_env_learning_curve.png}
    % \includegraphics[width=\textwidth]{figures/single_env/top/single_env_top.png}
    \includegraphics[width=0.28\textwidth]{figures/iqm-Single2.pdf}%
       \vline height 75pt depth 0 pt width 0.8 pt
    \includegraphics[width=0.72\textwidth]{figures/Continual_Single2.pdf}%
    \caption{\textbf{Left:} Aggregate Interquantile Mean \citep{agarwal2021deep} of scores. \textbf{Right} Comparison of different models and routers on the single environment setup. We report the mean of the normalised scores for 3 Atari games. All games run with 10 independent seeds, shaded areas representing the standard error. We normalise performance according to the single environment results reported in \citet{jesson2023relu}. BigMoE improves performance over the baseline, especially due to performance improvements in Asterix.\vspace{-5mm}}
    \label{fig:single_env_top}
\end{figure*}

\subsection{Single Environment}
% Some evidence that BigMoE with SoftMoE helps performance
Despite the clear improvements from CRL and MTRL, there are no significant performance improvements in the single environment setting across all games. However, \bigmoe improves over the baseline in Asterix, while performing worse in Breakout, as shown in \autoref{fig:single_env_top} and \autoref{tab:single_env}, suggesting that MoEs might be beneficial in specific types of environments. Note that adding gradient information did not affect performance (see \autoref{fig:single_env_vanilla}).

\subsection{Actor Critic Ablations}
By default, we use MoE modules in the actor and the critic. In Figure \ref{fig:crl_ac}, \ref{fig:mtrl_ac}, and \ref{fig:single_env_ac}, and Table \ref{tab:crl_ac}, \ref{tab:mtrl_ac}, and \ref{tab:single_env_ac} we show that using MoEs in both is beneficial in CRL, MTRL, and the single environment setting. The results suggest that the using an MoE in the actor provides more benefits than using it in the critic, and the combination of both adds additional benefits

\subsection{}{Order Ablation}
To test whether the order in CRL or MTRL made a difference, we train Ast$\rightarrow$ BO $\rightarrow$ SI instead. We report the ablations in \autoref{fig:mtrl_order} and \autoref{fig:crl_order}. The order did affect performance in both cases (see \autoref{tab:crl_order} and \autoref{tab:mtrl_order}), though the conclusion stays the same.

% Analyse specialisation again

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
Game & Big-SoftMoE & Baseline & Big-Hardcoded & Big-TopK \\
\hline
SI & 0.98 \pm 0.01 & 0.95 \pm 0.01 & 0.94 \pm 0.01 & 0.90 \pm 0.01 \\
BO & 0.54 \pm 0.09 & 0.66 \pm 0.08 & 0.52 \pm 0.07 & 0.54 \pm 0.07 \\
Ast & 0.67 \pm 0.03 & 0.58 \pm 0.03 & 0.57 \pm 0.03 & 0.32 \pm 0.01 \\
\hline
Total & \textbf{0.73} \pm 0.06 & \textbf{0.73} \pm 0.05 & \textbf{0.67} \pm 0.05 & 0.59 \pm 0.04 \\
\hline
\end{tabular}
\caption{Single environment: Normalised Performance of algorithms across games with average total performance. We normalise performance according to the single environment results reported in \citet{jesson2023relu}. We do not achieve the same performance as we use smaller networks due to computational limits.}
\label{tab:single_env}
\end{table}


\section{Related Work}
% We want to investigate if MoEs help with some of the many shortcomings of current Deep RL techniques, such as capacity loss and catastrophic forgetting. Next, we will provide an overview of the settings and methods that related work proposed to address said problems.
%
% Shortcomings of RL
\paragraph{Parameter Efficiency in Deep RL.} The challenge of achieving parameter efficiency in deep Reinforcement Learning (RL) is closely tied to the issue of underutilized parameters.
The latter was highlighed by \citet{sokar2023dormant} in a form of dormant neurons: the authors reveal that during online training an increasing number of neurons become inactive. A similar phenomena was observed in offline RL by \citet{gulcehre2022empirical}.
%Recent studies highlight that RL networks often do not fully utilize their parameters, with findings from \citet{sokar2023dormant} revealing a trend of increasing number of inactive neurons during online training, a phenomenon similar to the one observed in offline RL by \citet{gulcehre2022empirical}. 
Parameter underutilization was also observed in terms of achievable sparsity.
\citet{arnob2021single} demonstrate that in offline RL up to 95\% of network parameters can be pruned at initialization without impacting performance. 
Further, several studies have shown that performance can be enhanced through periodic network weight resets \citep{igl2020transient, dohare2021continual, nikishin2022primacy, doro2022sample, sokar2023dormant, schwarzer23bbf}, and that RL networks can maintain performance even when trained with a high degree of sparsity (approximately 90\%) \citep{tan2022rlx2, sokar2022dynamic, graesser2022state, obando2024deep}. 
These findings underscore the need for methods that more effectively leverage network parameters in RL training. Our work explores the use of Mixture of Experts (MoEs) for policy gradient methods, demonstrating significant reductions in dormant neurons across various tasks and network architectures.

\paragraph{Addressing Catastrophic Forgetting.} Catastrophic forgetting refers to the phenomenon in which a neural network loses previously learned information when it is trained on new tasks. RL's vulnerability to catastrophic forgetting is well-documented \citep{kirkpatrick2017overcoming,Atkinson_2021,khetarpal2022towards}. While methods like occasional weight resets have shown promise \citep{abbas2023loss}, our work explores the potential benefits of MoEs within a Continual RL setting as a way to mitigate forgetting.
%Recent work has shown that DRL suffers from issues such as catastrophic forgetting. \citet{abbas2023loss} address catastrophic forgetting by occasionally resetting the network weights. In contrast, our work uses the Continual RL setting as a test bed to investigate potential benefits of MoEs for DRL.

\paragraph{Multi-Task Reinforcement Learning (MTRL).}
MTRL seeks to develop agents capable of mastering diverse skills across multiple tasks
%MTRL addresses the challenge of equipping agents with versatile skills that can be applied across a broad spectrum of problems.
Representation sharing is crucial for identifying and leveraging the distinct and shared attributes of various tasks \citep{calandriello2014sparse,devin2017learning,yang2020multi,sun2022paco,deramo2024sharing}. 
However, the quest to learn a comprehensive set of diverse representations capturing multiple tasks remains a significant, unresolved challenge. 
%In contrast to previous work , 
In this work, we instead use MTRL to evaluate potential benefits of MoEs for policy gradient-based DRL.
%and do not propose a novel method designed explicitly for MTRL.

% Continual RL
\paragraph{Continual (Lifelong) Reinforcement Learning.}
Continual RL aims to create agents capable of continuously learning from multiple tasks without forgetting. 
Standard DRL often struggles in these settings \citep{khetarpal2022towards}, prompting exploration of techniques such as weight resets \citep{abbas2023loss}.  
Our work investigates how MoEs might offer advantages under continual learning conditions.
%Continual RL is a paradigm that extends beyond the conventional frameworks of Reinforcement Learning (RL) by focusing on the development of agents capable of learning from a continuous stream of experiences across multiple tasks, without forgetting previously acquired knowledge. It's been shown that standard DRL falls short in continual RL settings \citep{khetarpal2022towards}. For example, \citet{abbas2023loss} investigate if resetting the weights throughout training helps performance. In contrast, our work investigates the benefits of MoEs in Continual RL.

% MoEs in general
\paragraph{Mixture of Experts (MoEs).}
Introduced by \citet{jacobs1991adaptive}, MoEs have revolutionized large-scale language models primarily due to their modular design, which supports distributed training and enhances parameter efficiency during inference \citep{lepikhin2020gshard, fedus2022switch}. 
%MoEs were initially introduced by \citet{jacobs1991adaptive} and have since played a pivotal role in the scaling of language models to the trillion-parameter mark, primarily due to their modular design, which supports distributed training and enhances parameter efficiency during inference \citep{lepikhin2020gshard, fedus2022switch}. 
These models have not only achieved remarkable success in the realm of natural language processing but have also been extensively applied in the field of computer vision \citep{ yang2019condconv, wang2020deep, abbas2020biased, pavlitskaya2020using}. In computer vision, MoEs have facilitated the expansion of vision transformers to billions of parameters, concurrently halving the computational cost at inference \citep{riquelme2021scaling}, enhancing vision-based continual learning \citep{lee2019neural}, and addressing multi-task challenges \citep{fan2022m3vit}. Beyond these applications, MoEs have shown significant benefits in transfer and multi-task learning scenarios, for instance, by assigning experts to specific sub-problems \citep{puigcerver2023sparse, chen2023mod, ye2023taskexpert}, or by improving the statistical performance of routers \citep{hazimeh2021dselect}.

% MoEs in RL (bagging, mixing policies, policy representations)
\paragraph{MoEs in RL.}
MoEs and other related techniques, such as ensembles, have been previously studied in DRL. Ensembles are often used to represent the policy \citep{anschel2016deep, lan2020maxmin, agarwal2020optimistic, peer2021ensemble, chen2021randomized, an2021uncertainty, wu2021aggressive, liang2022reducing} or to predict model dynamics \citep{shyam2019model, chua2018deep, kurutach2018model}. Most closely related to ensembling is our BigMoE architecture, where each expert is a full model. \citet{fan2023learnable} could be interpreted as using multiple meta-controllers as routers for BigMoE and then ensembling the resulting policy. In contrast to our work, they do not investigate different MoE architectures and rely on population-based training. MoEs in DRL have also been investigated in the past \citep{ren2021probabilistic, hendawy2024multitask, akrour2021continuous}, but based on the previous definition of MoE, closely related to ensembling, and not the more recent interpretation of MoEs in LLMs. 

\section{Conclusion}

% Switching for continual RL is unsolved, Hardcoded Router shows promising results
The challenge of task switching in Continual Reinforcement Learning (CRL) remains largely unresolved. However, the Hardcoded Router variant has shown promising results, indicating a potential pathway towards more effective strategies for managing task transitions within this context. This approach stands out for its ability to provide a structured mechanism for switching between tasks, offering a glimmer of hope in addressing one of CRL's most persistent challenges.

% SoftMoE do not provide performance benefits for MTRL out of the gate
In the Multi-Task Reinforcement Learning (MTRL) setting, applying Hardcoded Router does not yield performance advantages. The expectation that SoftMoE might enhance task switching and learning efficiency in MTRL still needs to be met. This finding prompts a deeper exploration into the conditions under which SoftMoE can be effectively leveraged within MTRL frameworks.

% BigMoE with SoftMoE shows promising results on some tasks and seems to transfer to single environment setting
The combination of BigMoE with SoftMoE, however, unveils promising results in specific tasks, suggesting a nuanced relationship between MoE configurations and task performance. Notably, this combination demonstrates a capacity to improve outcomes in specific MTRL scenarios and shows potential for applicability in single-environment settings. This versatility highlights the importance of further investigating MoE configurations to uncover the mechanisms driving their success across different learning contexts.

% TopKRouter struggles across the board.
Conversely, the TopKRouter faces challenges consistently across various tasks. Its struggle to perform effectively underscores the complexities involved in designing routers that can adeptly manage the distribution of tasks among experts. The difficulties encountered by the TopKRouter reflect broader challenges in optimizing task routing mechanisms within MoE models, reaffirming the need for continued innovation and experimentation in this area.
 

\subsubsection*{Broader Impact Statement}
\label{sec:broaderImpact}
This paper introduces research aimed at pushing the boundaries of Machine Learning, with a particular focus on reinforcement learning. Our work holds various potential societal implications, although we refrain from singling out specific ones for emphasis in this context. 

% \subsubsection*{Acknowledgments}
% \label{sec:ack}
% Use unnumbered third level headings for the acknowledgments. All acknowledgments, including those to funding agencies, go at the end of the paper. Only add this information once your submission is accepted and deanonymized. 
